Face Deepfakes -- A Comprehensive Review

In recent years, remarkable advancements in deep-fake generation technology have led to unprecedented leaps in its realism and capabilities. Despite these advances, we observe a notable lack of structured and deep analysis deepfake technology. The principal aim of this survey is to contribute a thorough theoretical analysis of state-of-the-art face deepfake generation and detection methods. Furthermore, we provide a coherent and systematic evaluation of the implications of deepfakes on face biometric recognition approaches. In addition, we outline key applications of face deepfake technology, elucidating both positive and negative applications of the technology, provide a detailed discussion regarding the gaps in existing research, and propose key research directions for further investigation.

==> tex/fullbody.tex <==
\section{Full-body Deepfakes}
\label{sec:fullbody_deepfakes}

The term "deepfake" refers to synthetic media in which a person in an existing image or video is replaced with someone else's likeness using artificial intelligence. Full-body deepfakes are advanced synthetic media creations that use deep learning algorithms to generate realistic videos of a person's entire body. Unlike traditional deepfakes that focus on facial manipulation, full-body deepfakes replicate gestures, movements, and postures, creating an illusion of a person performing actions they never did. Even though full-body deepfakes are not extensively explored as a separate field of study, techniques such as image animation, which uses deep learning to bring static images to life by inferring realistic motions, can be considered part of deepfakes. This technology uses models such as GANs and motion transfer algorithms to create a single image based on the motion patterns derived from a driving video. This process can make a person in a still photo appear to move, speak, or perform various actions, creating highly engaging and dynamic visuals resulting in deepfakes. 

\subsection{Performance Evaluation in Full-body Animation}
\label{sub:fullbody_metrics}

In evaluating motion transfer from the driving video to the source video in most state-of-the-art methods, both quantitative and qualitative analyses are employed, allowing a comprehensive assessment of the effectiveness of the motion transfer process. Quantitative analysis involves the use of various metrics to assess performance, and such metrics are listed below.  

\paragraph{L1 Distance ($L_1$)}

The L1 distance can be used to quantify the difference between the pixel values of the two videos frame by frame and can be calculated as in Equation \ref{eq:fullbody_l1} where $I_1$, $I_2$, $m$, $n$, and $T$ refer to ground-truth frame, generated frame, width of the frame, height of the frame image and number of frames in the video respectively.

\begin{equation}
    L_1 = \Sigma_{t=1}^T \Sigma_{i=1}^m \Sigma_{j=1}^n | I_1 (i,j) - I_2 (i,j) |
    \label{eq:fullbody_l1}
\end{equation}


\paragraph{Average Keypoint Distance (AKD)}

The average key point distance in animation generation is a measure used to evaluate how accurately the generated animation matches the ground truth regarding specific key points, such as facial landmarks, joint positions, or other significant points. First, the key points which are represented as coordinates in the image space are extracted from both the ground truth and the generated animation frame. The Euclidean distance is calculated between the corresponding key points of ground truth and generated images, followed by averaging over all the pairs. This metric provides a meaningful way to assess the quality of the generated animation by focusing on how well it replicates the key structural features of the ground truth. $AKD$ can be calculated as illustrated in Equation \ref{eq:fullbody_akd} where $T$, $N$ and $K$ refer to the number of frames in the video, the number of key points in a frame and the key points ($K(x,y)$) respectively.

\begin{equation}
    AKD = \frac{1}{T} \Sigma_{t=1}^T \frac{1}{N} \Sigma_{i=1}^N || K_1^t(i) - K_2^t(i)||
    \label{eq:fullbody_akd}
\end{equation}

\paragraph{Missing Keypoint Rate (MKR)}

The Missing keypoint rate (MKR) in animation generation is a metric that quantifies the frequency at which key points are not detected or generated in the animation compared to the ground truth. First, the key points are detected in both ground truth and generated images, and a threshold $d_{th}$ is used to determine whether a key point is detected or not. The key point is considered missing if the distance between the ground truth key point and the generated key point exceeds $d_{th}$. Then, the number of key points in the ground truth that do not have a corresponding generated key point within the threshold distance is counted over all the frames and averaged to obtain $MKR$ (refer to Equation \ref{eq:fullbody_mkr}). 

\begin{equation}
    MKR = \frac{1}{N \times T} (\Sigma_{t=1}^T \Sigma_{i=1}^N ||K_1^t(i) - K_1^t(i) || > d_{th})
    \label{eq:fullbody_mkr}
\end{equation}

\paragraph{Average Euclidean Distance (AED)}

The Average Euclidean Distance (AED) calculates the average Euclidean distance in feature embedding between the ground truth representation and the generated video. The chosen feature embedding assesses how well the identity is maintained. Public re-identification networks for bodies extract identity from reconstructed and ground truth frame pairs and then compute the mean L2 norm of their difference across all pairs. \cite{siarohin2021motion}.

\subsubsection{Datasets for Full-body Deepfake (Video Animation) Generation}

Most state-of-the-art methods in the next section are evaluated using the Tai-Chi-HD and TED-Talks datasets. The Tai-Chi-HD dataset comprises 3048 (2884 in \cite{guo2024human}) and 285 video chunks for training and testing, extracted from 252 training and 28 testing videos, respectively \cite{hong2022qs, siarohin2019first}. The video length varies from 128 to 1024 frames \cite{siarohin2019first}. The TED-Talks dataset consists of videos from TED talks available on YouTube, with 1132 training videos and 131 test videos (1255 in \cite{tao2022motion}) \cite{guo2024human}. The number of frames per video ranges from 64 to 1024 \cite{guo2024human, zhao2022thin, siarohin2021motion}. The slight variations in dataset distributions mentioned above might have caused differences in the performances of different state-of-the-art models, as shown in Table \ref{tab:fullbodydatasets}. Furthermore, a low-resolution Tai-Chi dataset \cite{tulyakov2018mocogan} was also used in earlier evaluations which consisted of 4500 tai-chi video clips split into 3288 and 822 videos for training and testing sets respectively. The video length of the Tai-Chi dataset varied from 32 to 100 frames \cite{siarohin2019animating}. The Tai-Chi dataset consisted of low-resolution frames (64 $\times$ 64), while Tai-Chi-HD included frames with resolutions of 256 $\times$ 256 and 512 $\times$ 512. The TedTalks dataset mainly utilized frames with a resolution of 512 $\times$ 512.

\subsection{Full-body Deepfake (Video Animation) Generation}
\label{subsec:fullbody_generation}

Motion transfer is a key technique in creating full-body deepfake videos. It involves taking the movements or poses from one person (the "driving source") and applying them to another person (the "target" or "source subject") so that the target subject mimics the exact movements of the driving subject. This is done while keeping the appearance of the target subject, essentially allowing one person’s body movements to be applied to another person. Recent advancements in deep learning, particularly in motion transfer, pose estimation, and video synthesis, have led to the development of models capable of generating high-quality full-body deepfake videos. Two commonly used datasets for full-body deepfake generation and motion transfer are the TaiChiHD dataset and the TED Talks dataset. The TaiChiHD dataset is primarily used for generating full-body animations that capture precise, fluid human motions, such as Tai Chi movements. It focuses on complex poses and transitions between them. Models trained on TaiChiHD can learn to transfer precise body movements from one individual to another, ensuring that synthesized videos maintain the accuracy of the poses and gestures while adapting the appearance of the subject. The TEDTalks dataset can be used to extract and model the dynamic body language and physical gestures exhibited by speakers. These movements can then be transferred to another target subject, creating a video where the target mimics the gestures and body language of the TEDTalks speaker. Some state-of-the-art techniques in motion transfer methods are given in Table \ref{tab:fullbodydatasets} (summarised in Figure \ref{fig:taichihd} and \ref{fig:tedtalks}) and are discussed in Section \ref{subsubsec:fullbody_gen}.

\subsubsection{Literature Review on Full Body Deepfake Generation}
\label{subsubsec:fullbody_gen}

Monkey-Net (MOviNg KEYpoints) \cite{siarohin2019animating} is a groundbreaking model used for motion transfer and creating realistic deepfake animations. It transfers motion from a driving video to a target image to create animations using deep learning. The network included a keypoint detector trained to extract object keypoints, a dense motion prediction network for generating dense heatmaps from sparse keypoints to better encode motion, and a motion transfer network that uses the motion heatmaps and appearance information from the input image to create the output frames. Siarohin \textit{et al} \cite{siarohin2021motion} introduced a new approach for motion transfer (MRAA), which does not rely on keypoint detectors. They developed a network that can identify object parts, track them in a video, and infer their motions based on their principal axes. Unlike previous methods that used keypoint detectors, this approach focuses on extracting meaningful and consistent regions corresponding to semantically relevant and distinct object parts easily detected in the video frames. To separate foreground from background, they incorporated an additional affine transformation to model non-object-related global motion. They also disentangled the shape and pose of objects in the region space to facilitate animation and prevent the leakage of the driving object's shape. Since MRAA uses local affine transformations near the keypoints to estimate the motion, the temporal continuity of the reconstructed video depends on the smoothness of the
keypoints change. If the location of the key points in two adjacent frames changes greatly, it can cause pixel jitter \cite{zhao2022thin}. In the TPS-MM method proposed by Zhao \textit{et al.}, the use of Thin-Plate-Spline (TPS) motion estimation alleviated previous issues by generating each transformation using multiple keypoints, thus increasing the robustness of motion estimation. Before the TPS-MM method \cite{zhao2022thin}, motion transfer on arbitrary objects was mainly conducted using unsupervised methods without prior knowledge. However, these unsupervised methods often failed when there was a large pose gap between the objects in the source and driving images. As a solution, TPS-MM proposes an end-to-end unsupervised motion transfer framework that utilizes thin-plate spline motion estimation to create a more flexible optical flow, which warps the feature maps of the source image to the feature domain of the driving image. Additionally, to restore the missing regions, they propose multi-resolution occlusion masks to achieve more effective feature fusion. Despite significant advancements in the field of motion transfer, challenges such as distorted limbs and missing semantics persist due to the complex representation of motion and the unknown correspondence between human bodies. To address these challenges, Guo \textit{et al.} \cite{guo2024human} proposed a novel, semantically guided, unsupervised method of motion transfer that utilizes semantic information to model motion and appearance. This approach involved utilizing a pre-trained human parsing network to encode rich foreground semantic information, enabling the generation of fine details. Additionally, an attention-based network layer was proposed to learn the semantic region's correspondence between human bodies, guiding the network in selecting appropriate input features and ultimately leading to more accurate results.

\begin{table*}[htbp]
\caption{\textcolor{black}{State-of-the-art Video Animation Generation Methods (Video reconstruction). We have highlighted the performance of each method as given in the original paper. However, a few evaluation metrics on the TedTalks dataset and all FID values were referred from HIA-SG \cite{guo2024human}, and referred through $^\dagger$. $^{\ast}$ represents performance on Tai-Chi dataset.}}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|P{95pt}|P{27pt}|P{27pt}|P{27pt}|P{27pt}|P{27pt}||P{27pt}|P{27pt}|P{27pt}|P{27pt}|P{27pt}|P{27pt}|}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c||}{TaiChiHD} & \multicolumn{5}{c|}{TedTalk}\\\cline{2-11}
 & $L_1$ & $AKD$ & $MKR$ & $AED$ & $FID$ & $L_1$ & $AKD$ & $MKR$ & $AED$ & $FID$ \\\hline\hline
HIA-SG \cite{guo2024human} & 0.049 & 4.34 & 0.016 &  0.154 & 25.57$^\dagger$ & 0.030 & 3.38 &  0.007 & 0.138 & 25.78$^\dagger$\\\hline
TPS-MM \cite{zhao2022thin} & 0.045 & 4.57 & 0.018 &  0.151 & 24.29$^\dagger$ & 0.027 & 3.39 &  0.007 & 0.124 &  23.28$^\dagger$ \\\hline
Motion Transformer \cite{tao2022motion} & 0.045 & 4.670 & 0.021 & 0.148 & - & 0.026 & 3.456 & 0.007 & 0.113 & - \\\hline
QS-Craft \cite{hong2022qs} & - & 4.61 & 0.017 & - & 25.064 & - & - & - & - & - \\\hline
FOMM \cite{siarohin2019first} & 0.063 & 6.862 & 0.036 & 0.179 & 28.08$^\dagger$ & 0.033$^\dagger$ & 7.07$^\dagger$ &  0.014$^\dagger$ &  0.163$^\dagger$ & 29.87$^\dagger$\\\hline
MRAA \cite{siarohin2021motion} &  0.047 & 5.58 & 0.027 & 0.152 & 25.74$^\dagger$ & 0.026 & 4.01 & 0.012 &  0.116 & 22.54$^\dagger$\\\hline
Monkey-Net \cite{siarohin2021motion} & 0.077 & 10.80 & 0.059 & 0.228 & - & - & - & - & - & - \\\hline
Monkey-Net$^{\ast}$ \cite{siarohin2019animating} & 0.050$^{\ast}$ & 2.53$^{\ast}$ & \textcolor{black}{17.4}$^{\ast}$ & 0.21$^{\ast}$ & - & - & - & - & - & - \\\hline
\end{tabular}}
\label{tab:fullbodydatasets}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures_new/TaiChi.pdf}
    \caption{\textcolor{black}{Performance variation of recent state-of-the-art methods in motion transfer to create full body deepfakes on Tai-Chi-HD dataset}}
    \label{fig:taichihd}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures_new/TedTalk.pdf}
    \caption{\textcolor{black}{Performance variation of recent state-of-the-art methods in motion transfer to create full body deepfakes on TedTalks dataset}}
    \label{fig:tedtalks}
\end{figure}


\textcolor{black}{Motion transfer technology is rapidly advancing, enabling the creation of highly realistic full-body deepfake animations by mapping motion from a video onto a static image. At its core, motion transfer involves generating representations of movement that can capture complex human motions and expressions, allowing animations to synchronize seamlessly with the source video. This technology synthesizes both appearance and motion in increasingly smooth and lifelike ways, facilitating the production of convincing animated content. By identifying key body parts and tracking their movements, these systems replicate subtle details in a subject’s posture, gestures, and interactions while maintaining coherence across frames. However, this level of realism raises important ethical questions regarding deepfake content. The ability to produce highly believable full-body deepfakes that mimic specific individuals can blur the line between reality and artificial content in media. As a result, the future of motion transfer technology in deepfakes will likely involve balancing creative applications with ethical considerations. Society must navigate the implications of increasingly realistic virtual representations on privacy, trust, and the authenticity of media.}

\subsubsection{Literature Review on Full Body Deepfake Detection} 

To the best of our knowledge, currently there is no method to detect full-body deepfakes.

\subsection{Combating Full-body Deepfakes in Gait Biometrics}
Gait biometrics is recently being adapted into security surveillance applications such as identifying and tracking individuals from CCTV footage. Therefore, it is important to investigate whether full-body deepfakes are capable of maintaining a subject's gait biometric features when animating a still image of that particular subject. In the following subsection, we discuss the summary of the findings
of our evaluation, and a detailed discussion is provided in Sec.
IV of supplementary material.

\subsubsection{Efficacy of full-body deepfakes to fool gait biometrics systems} Table IV in Sec. IV of supplementary material demonstrates the viability of full-body deepfakes to fool gait recognition models. Specifically, we observe substantial vulnerability when synthesising normal walking patterns of the target subject. Therefore, it is important to address this limitation of gait recognition methods. lease refer to Sec. IV of supplementary
material for additional details regarding this evaluation.

\subsubsection{Measures for revealing true identity: }To the best of our knowledge, currently there is no method to reveal true identity from full-body deepfakes.


==> tex/multimodal.tex <==
% \newpage
\section{Multimodal Deepfakes}
\label{sec:multimodal_deepfakes_intro} 

The concept of multi-modality in deep learning involves integrating and processing data from various sources simultaneously. These sources can encompass text, images, audio, video, and sensor data. By leveraging different data types, multi-modal deep learning models can capture more comprehensive and diverse information, resulting in enhanced performance for tasks that require understanding the relationships between different data types \cite{gao2020survey, summaira2021recent, jabeen2023review}. In the realm of deepfakes, multi-modality entails using various types of data, such as images, audio, and video, to create highly realistic synthetic media that convincingly mimics real-world content, including visuals and sounds \cite{khalid2021fakeavceleb, hou2024polyglotfake}. Through aligning and synchronizing these modalities, deepfakes can produce seamless and coherent fake content, such as matching a person's lip movements to a different audio track or convincingly cloning their voice \cite{pei2024deepfake, prajwal2020lip, cheng2022videoretalking, lomnitz2020multimodal}. While this technology offers positive applications in entertainment, media, and education, such as creating special effects and developing realistic training simulations, it also poses significant ethical and security challenges \cite{pandey2021deepfakes}. These include the potential for misuse in misinformation, impersonation, and fraud. Detecting and preventing malicious deepfakes is a burgeoning area of research aimed at ensuring the responsible use of this powerful technology. As multi-modal deepfakes continue to evolve, it is crucial to balance innovation with ethical considerations to mitigate risks and maximize benefits \cite{khalid2021evaluation, liu2023magnifying, cheng2023voice}. In this section, we will investigate state-of-the-art methodologies for the generation (refer Section \ref{subsec:multimodal_generation}) and the detection of multi-modal deepfakes (refer Section \ref{subsec:multimodal_detection}). We will analyze the advanced and innovative techniques outlined in the existing literature, alongside the datasets utilized for deepfake detection and generation.

\subsection{Multimodal Deepfake Generation}
\label{subsec:multimodal_generation}

Combining audio and video deepfakes involves a sophisticated process of synchronizing lip movements with synthetic speech to produce seamless and coherent content \cite{liz2024generation}. This multi-modal approach, which integrates both visual and auditory elements, significantly enhances the realism of the generated media. By ensuring that the audio matches the lip movements and facial expressions perfectly, these deepfakes become more lifelike and convincing, making detection increasingly challenging \cite{hou2024polyglotfake}. Audio-visual multimodal deepfakes can be categorized into three main types based on the modality being faked \cite{khalid2021fakeavceleb}. This categorization helps in understanding the different ways in which deepfakes can manipulate audio and visual components to create convincing forgeries. Understanding these categories is important for recognizing and combating the potential misuse of deepfake technology.

\paragraph{Fake Video and Real Audio}
\label{para:multimodal_fakeV_realA}

Fake video and real audio deepfakes involve manipulating visual content while retaining the original audio, creating a synthetic video that depicts events or actions that never actually occurred. By keeping the original audio, which includes the true voice, tone, and speech patterns of the person, these deepfakes gain an added layer of credibility and can be particularly persuasive. The process of creating fake videos with real audio often involves altering the appearance, expressions, or actions of individuals in the video \cite{karras2019style, nirkin2019fsgan, korshunova2017fast}. For instance, face swapping \cite{korshunova2017fast} can replace the subject’s face with someone else's, or visual effects can be used to create entirely new scenes that seem authentic. The combination of real audio and fake video poses significant challenges for detection, as the genuine audio can make the fabricated visuals appear more believable. Detecting these deepfakes involves analyzing inconsistencies between the audio and video elements. Techniques such as temporal analysis of facial expressions, detecting unnatural movements, and scrutinizing visual artifacts are crucial \cite{kaur2020deepfakes, liu2023ti2net}.

\paragraph{Real Video and Fake Audio}
\label{para:multimodal_realV_fakeA}

In this type of deepfake, the video remains unaltered, while the audio is synthetically generated to mislead the audience about what is being said. This method generally involves using text-to-speech models and voice cloning techniques to create synthetic speech that closely mimics the vocal characteristics of a specific person \cite{deng2020unsupervised, kinnunen2017asvspoof, polyak2019tts}. By manipulating the audio, these deepfakes can make it seem like the person in the video is saying something they never actually said. This technique is particularly dangerous because the genuine video lends credibility to the fake audio, making it more convincing and harder to detect. Examples of using real video with fake audio include creating false news reports, tampering with evidence in legal cases, and producing deceitful content for political propaganda \cite{sankaranarayanan2021presidential}. Detecting such deepfakes requires a comprehensive analysis of audio-visual synchronization to identify discrepancies between lip movements and speech \cite{agarwal2020detecting}. Additionally, it demands the development of robust audio forensic techniques to scrutinize voice patterns and identify synthetic anomalies \cite{almutairi2022review}.

\paragraph{Fake Video and Fake Audio}
\label{para:multimodal_fakeV_fakeA}

These deepfakes manipulate visual content to depict events or actions that never occurred, while also synthesizing audio to accompany the fabricated visuals.  This allows for a wider range of possible sample alterations and a variety of manipulation techniques. For example, a deepfake could depict a person giving a speech they never delivered, with the voice and the video being entirely fabricated. Achieving realism in both modalities requires training models on large datasets of real audio and video to learn the nuances of human speech, facial expressions, and body movements. The challenge lies in creating seamless synchronization between the audio and video components to make the deepfake indistinguishable from genuine content. Furthermore, standardized multimodal deepfake datasets serve as benchmarks for evaluating the performance of detection algorithms \cite{dolhansky2020deepfake, khalid2021fakeavceleb, hou2024polyglotfake}. They offer a common ground for researchers to compare different approaches, facilitating the identification of the most effective methods for detecting deepfakes \cite{liu2023magnifying, cheng2023voice, feng2023self}. This benchmarking is vital for pushing the boundaries of deepfake detection technology, ensuring that the algorithms can generalize well across different types of deepfakes and are not limited to specific scenarios or formats.

\subsection{Multimodal Deepfake Detection Datasets}
\label{subsec:multimodal_datasets}

Multimodal deepfake datasets are crucial for advancing the understanding and detection of deepfakes, which involve the manipulation of multiple types of data such as audio, video, and text to create convincingly fake content. These datasets offer diverse examples of synthetic media that combine various modalities, accurately reflecting the complex, real-world scenarios where deepfakes are likely to be encountered. This diversity is indispensable for training sophisticated detection techniques, primarily deep learning-based networks, to recognize and detect deepfakes across various scenarios and formats. By including examples that span different combinations of audio, video, and text manipulations, multimodal datasets allow researchers to develop and refine algorithms that can analyze the consistency and coherence between these modalities.

Multimodal deepfake datasets are essential for advancing both the understanding and detection of deepfakes, which involve manipulating multiple types of data, such as audio and video, to create compelling fake content. These provide diverse examples of synthetic media, combining various modalities like audio, video, and text reflecting real-world scenarios where deepfakes are likely to be used. This diversity is essential for training sophisticated detection techniques (mainly deep learning-based networks) to recognize and detect deepfakes across different scenarios and formats. These multimodal datasets enable researchers to develop algorithms that analyze the consistency and coherence between modalities. Furthermore, standardized multimodal deepfake datasets offer benchmarks for evaluating the performance of detection algorithms. They provide a common ground for comparing different approaches and identifying the most effective methods for detecting multimodal deepfakes.

\begin{table*}[htbp]
\caption{\textcolor{black}{Multimodal Deepfake Datasets}}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|P{67pt}|P{42pt}|P{40pt}|P{35pt}|P{35pt}|P{100pt}|P{100pt}|}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Multilingual} & \multirow{2}{*}{Subjects} & \multicolumn{2}{c|}{Samples} & \multicolumn{2}{c|}{Manipulation Techniques} \\\cline{4-7}
&  &  & Real & Fake & Video & Audio\\\hline\hline
DFDC \cite{dolhansky2020deepfake} & No  & 960 & 104,500 & 23,654 & DFAE, MM/NN face swap, NTH, FSGAN \cite{nirkin2019fsgan}, StyleGAN \cite{karras2019style} & TTS-Skins \cite{polyak2019tts}\\\hline
FakeAVCeleb \cite{khalid2021fakeavceleb} & No  & 500 & 500 & 19,500 & FaceSwap \cite{korshunova2017fast}, Wav2Lip \cite{prajwal2020lip}, FSGAN & SV2TTS \cite{jia2018transfer}\\\hline
VideoSham \cite{mittal2023video} & No & - & \textcolor{black}{413} & \textcolor{black}{413} & \multicolumn{2}{c|}{Manual manipulations by professional video editors (6 types)} \\\hline
PDD \cite{sankaranarayanan2021presidential} & No & 2 & 16 & 16 & Wav2Lip & Manipulated content recorded by voice actors \\\hline
LAV-DF \cite{cai2022you} & No & 153 & 36,431 & 99,873 & Wav2Lip & SV2TTS \\\hline
MMDFD \cite{asha2023mmdfd} & No  & 50 & 1,500 & 5,000 & FaceSwap, FSGAN, Wav2Lip, DeepFaceLab \cite{perov2020deepfacelab} & SV2TTS (AurisAI \cite{aurisaiAurisFree} for Text)\\\hline
DefakeAVMiT \cite{10081373} & No  & 43 & \multicolumn{2}{c|}{6,480} & FaceSwap, DeepFaceLab, EVP \cite{ji2021audio}, Wav2Lip, PC-AVS \cite{zhou2021pose}  & SV2TTS, Voice Replay \cite{kinnunen2017asvspoof}, AV exemplar autoencoders \cite{deng2020unsupervised} \\\hline
PolyGlotFake \cite{hou2024polyglotfake} & Yes  & 766 & 766 & 14,472 & VideoRetalking \cite{cheng2022videoretalking}, Wav2Lip & XTTS \cite{Gölge2024coqui}, Bark \cite{Kucsko2024suno} + FreeVC \cite{li2023freevc}, Tacotron \cite{wang2017tacotron} + FreeVC, MicrosoftTTS \cite{microsoftTextSpeech} +FreeVC, Vall-E-X \cite{wang2023neural}\\\hline
\end{tabular}}
\label{tab:multimodal_datasets}
\end{table*}

As illustrated in Table \ref{tab:multimodal_datasets}, the manipulation of modalities to generate multimodal deepfakes was accomplished using state-of-the-art deepfake generation techniques available at the time of the dataset release. The quality of the synthetic content is contingent upon the strengths and limitations of these techniques. Advances in sophisticated deep learning methodologies over time have yielded increasingly realistic fake content. Consequently, the techniques employed for multimodal deepfake generation are further elaborated in Section \ref{subsec:multimodal_generation}.

\subsection{Multimodal Deepfake Generation}
\label{subsec:multimodal_generation}

In the following section, we will delve into the latest and most widely utilized techniques for producing synthetic audio-visual content by synchronizing lip and/or face movements, drawing from state-of-the-art research in the field.

\paragraph{LipGAN}
\label{para:multimodal_lipgan}

Prajwal \textit{et al.} \cite{kr2019towards} proposed a GAN-based lip synchronization model called LipGAN. This model is capable of handling faces in random poses without the need for realignment to a template pose. Furthermore, LipGAN enables the generation of realistic talking face videos through an automated pipeline for face-to-face translation from any audio, without dependence on language.

\paragraph{Wav2Lip}
\label{para:multimodal_wav2lip}

Most state-of-the-art methods excel at generating accurate lip movements for static images or videos of specific individuals seen during the training phase. However, these methods often fail to accurately morph lip movements for arbitrary identities in dynamic, unconstrained talking face videos, resulting in significant portions of the video being out-of-sync with the new audio. As discussed by Prajwal et al. in \cite{\cite{prajwal2020lip}}, this failure can be primarily attributed to limitations in both training objectives (i.e., loss functions used) and lip-sync discriminators. Typically, the face reconstruction loss is computed for the detected facial region to ensure correct pose generation and identity preservation. However, the lip region constitutes a very small proportion of the face region (or the entire frame), causing the total reconstruction loss (often L1 distance) to be less impacted by the lip region due to its limited spatial extent. This can adversely affect the learning process, where the reconstruction of the surrounding image is prioritized over the lip region. To address this issue, specific discriminators, such as those used in LipGAN \cite{kr2019towards}, are employed to evaluate lip-sync accuracy. Prajwal et al. \cite{prajwal2020lip} emphasized the importance of short temporal context in detecting lip-sync discrepancies and incorporated this concept into the development of the Wav2Lip framework. They demonstrated that considering a short temporal context significantly improves lip-sync accuracy. Additionally, they noted that introducing artifacts such as pose variations during GAN training can negatively impact lip-sync performance. This degradation occurs because the discriminator may fail to focus on the correspondence between the video and lip movements, underscoring the need for discriminators specifically designed to evaluate lip-sync quality. Prajwal \textit{et al.} utilises a customised SyncNet-based \cite{chung2017out} discriminator to mitigate the limitations mentioned above, which is substantially more accurate than the previous methodologies. Furthermore, to increase the quality of the morphed regions in the reconstructed images, they have also utilised a visual-quality discriminator. This technique has been used by most of the above multimodal datasets to generate faked audio-visual content.

\paragraph{FaceRetalking}
\label{para:multimodal_faceretalking}

Cheng \textit{et al.} \cite{cheng2022videoretalking} highlighted that the state-of-the-art techniques often omit the original lip motion changes or retiming the background to avoid unnatural movements between the head pose and lip \cite{prajwal2020lip, song2022everybody}. However, in the FaceRatalking method, the lower half face (not only the lip) Cheng \textit{et al.} emphasized that existing state-of-the-art approaches often overlook authentic lip motion alterations or adjust the background timing to prevent unnatural movements between head pose and lip motion. In contrast, the FaceRatalking technique not only modifies the lip region but also encompasses editing of the entire lower half of the face, incorporating facial movements through an innovative face reenactment process. Additionally, they identified an information leakage in conditional in-painting-based methods when the original frame was utilized as the conditional image for lip synchronization. To remedy this, they introduced a semantic-guided reenactment network to alter the expression of the entire lower half of the face, producing an enriched frame with a consistent expression, which then served as the basis for subsequent lip synthesis. The lip synthesis network in the FaceRetalking approach incorporates a conditional inpainting-inspired network \cite{prajwal2020lip}. This network leverages pre-processed frames from the face reenactment network as the identity and structure reference, along with the audio and the masked original frames as the condition resulting in a highly effective method for synthesizing a lip-syncing video based on the input audio. They argued that even though the synthesized videos accurately depict lip movements, the visual quality is limited due to low-resolution training data. To tackle this issue, they developed an identity-preserving face enhancement network to improve output quality through progressive training. When compared to Wav2Lip \cite{prajwal2020lip} which mainly focuses only on lip synchronization, FaceRetalking provides a broader facial synthesis that includes expressions and head movements, enabling more realistic fake content.

\paragraph{Diff2Lip}
\label{para:multimodal_diff2lip}

In their work, Mukhopadhyay \textit{et al.} \cite{mukhopadhyay2024diff2lip} proposed Diff2Lip, which is an audio-conditioned diffusion model used for inpainting producing precise and natural lip sync by focusing on the fine details of lip movements. This model can achieve lip synchronization in real-world scenarios while preserving identity, pose, emotions, and image quality. The Diff2Lip model takes three inputs: a masked input frame (providing pose context), a reference frame (containing identity and mouth region textures), and an audio frame (used to drive the lip shape). It then outputs the lip-synced mouth region. The multimodal conditional diffusion implemented in the model allows for a fine balance between all contextual input information, effectively avoiding lip-sync problems. However, when compared with the FaceRetalking model, the FaceRetalking may provide a better integrated facial performance, enhancing overall expressiveness and realism beyond just the lips. However, through the leverage of the diffusion process, Diff2Lip can enhance the naturalness and fluidity of lip movements over time compared to similar lip synthesis methods such as Wav2Lip.


\subsection{Performance Evaluation in Deepfake Generation}
\label{subsec:multimodal_lossfunc}


Performance evaluation is a critical step in multimodal deepfake generation, providing a comprehensive framework to ensure that the generated content is realistic, high-quality, coherent, and consistent across different modalities. Various performance evaluation metrics are employed in the literature, encompassing both application-specific and generalized measures. In this section, we discuss some of the most widely considered performance metrics and their roles in assessing the quality and consistency of multimodal deepfake generation models.

\paragraph{The Fréchet Inception Distance (FID)}

The Fréchet Inception Distance (FID) serves as a crucial metric for evaluating the quality of generated images \cite{nunn2021compound, singh2020using, yu2021artificial}. By comparing the feature distribution of generated images with real images, it provides valuable insights into both the fidelity and diversity of the generated images. Lower FID values signify higher similarity to real images, indicating superior quality. An FID of 0 implies that the generated images are indistinguishable from real images in terms of their feature distributions. However, the FID score is sensitive to the choice of feature extractor. The FID score can be calculated as in Equation \ref{eq:multimodal_fid} where $\mu_r$, $\mu_g$, $\Sigma_r$, $\Sigma_g$ and $T_r$ represent the mean of real image features, mean of generated image features, covariance or real image features, covariance of generated image features and Trace of the matrix respectively \cite{nunn2021compound}. 

\begin{equation}
    FID = ||\mu_r - \mu_g||^2 + Tr(\Sigma_r+\Sigma_g - 2(\Sigma_r\Sigma_g)^{0.5})
    \label{eq:multimodal_fid}
\end{equation}

\paragraph{Structural Similarity Index (SSIM)}

SSIM compares two images by analyzing their structure, luminance, and contrast. Its goal is to provide a more accurate measure of perceptual image quality compared to simpler metrics like Mean Squared Error (MSE). SSIM is specifically designed to take human perception into account when assessing image quality, making it a more reliable method \cite{sun2020landmark, dagar2022literature, husseini2023comprehensive}. It does not consider higher-order image statistics, which may be important for certain aspects of image quality. However, it's important to note that SSIM is a pixel-wise image similarity metric that compares two images and may not be the best choice for capturing variability in video generation \cite{shrivastava2021diverse}. The SSIM can be calculated as in Equation \ref{eq:multimodal_ssim} where $c_1$, and $c_2$ represent constants to stabilize the division with a weak denominator \cite{wang2004image}.

\begin{equation}
    SSIM(x,y) = \frac{(2\mu_x \mu_y + c_1)(2\sigma_{xy}+c_2}{(\mu_x^2+\mu_y^2+c1)(\sigma_x^2+\sigma_y^2+c_2)}
    \label{eq:multimodal_ssim}
\end{equation}

\paragraph{Lip Movement Distance (LMD)}

Lip Movement Distance (LMD) is an important metric used to assess how well the movement of lips matches the corresponding audio, especially in the context of creating deepfakes. It measures the spatial difference between the lip positions in the generated frames and the actual frames, providing a quantitative evaluation of the accuracy of lip movements to the spoken audio \cite{chen2018lip}. However, the accuracy of LMD depends on the reliability of the facial landmark detection model used to extract lip positions. Additionally, since LMD focuses on spatial alignment, it may not fully capture the temporal dynamics and smoothness of lip movements over time. The LMD over $N$ frames can be calculated as in Equation \ref{eq:multimodal_lmd} where $L_t^{gen}$, and $L_t^{gt}$ represent lip landmarks for the generated and ground truth images respectively \cite{chen2018lip}.

\begin{equation}
    LMD = \frac{1}{N} \Sigma_{t=1}^n ||L_t^{gen} - L_t^{gt}||
    \label{eq:multimodal_lmd}
\end{equation}

\paragraph{LSE-C and LSE-D}

LSE-C and LSE-D are two important metrics used to assess the performance of the Wav2Lip model \cite{prajwal2020lip}, which is used to achieve synchronisation of audio-manipulated talking face videos. This model ensures that the lip movements in a video align with the corresponding audio. The LSE-D error (Lip-Sync Error-Distance), measures the misalignment between audio and visual streams in terms of lip synchronization, and a lower LSE-D denotes a higher audio-visual match \cite{prajwal2020lip}. LSE-C (Lip-Sync Error-Confidence) is the confidence score. A higher score suggests a better audio-visual correlation and more accurate alignment of lip movements with audio. Prajwal \textit{et al.} calculated these error metrics based on SyncNet \cite{chung2017out} extracted features from both the audio and visual inputs where the visual features are typically derived from the region around the lips, while audio features are extracted from the corresponding audio segment. However, poor feature extraction can lead to inaccurate error measurement, and may not capture the naturalness of continuous speech synchronization. These losses have been widely used in later research to validate the performance of lip-speech synchronisation \cite{wang2022attention, zhang2022meta, lu2022visualtts}. 

\paragraph{Peak Signal-to-Noise Ratio (PSNR)}

PSNR, which stands for Peak Signal-to-Noise Ratio, is a metric used to measure the quality of a reconstructed or generated image in comparison to a reference image \cite{huang2020fakeretouch, huang2020fakepolisher, wang2021faketagger}. It quantifies the level of distortion or noise introduced during the generation process, with higher PSNR values indicating better quality and less distortion. PSNR is easy to compute and understand, unlike most other metrics, providing a straightforward measure of image and video quality. However, it's important to note that PSNR does not always align well with human visual perception, and high PSNR values do not guarantee that the image will look good to human observers. PSNR can be calculated as in Equation \ref{eq:multimodal_psnr} where $MAX$ and $MSE$ refer to the maximum pixel value (can be either 1 or 255 depending on whether the input image is in double-precision floating-point or 8-bit unsigned integer format) and the Mean Squared Error (MSE) between the reference video frame (or image) and the generated frame.

\begin{equation}
    MSE = \frac{\Sigma_{M,N}[I_1(m,n)-I_2(m,n)]^2}{M*N}
    \label{eq:multimodal_psnr}
\end{equation}

\begin{equation}
    PSNR = 10.log_{10} (\frac{MAX^2}{MSE})
    \label{eq:multimodal_psnr}
\end{equation}

% \paragraph{Lip Sync Error Rate (LSER)}

% Lip sync error rate is the measure of how often or to what extent the audio track of a video does not match up correctly with the visual track of the speaker's lip movements. Various techniques can be used to calculate this metric, all of which assess how well the created lip movements synchronize with the accompanying audio, ensuring that the visual and audio components are convincingly synchronized. 

The performance metrics mentioned above can be divided into two main categories: lip-sync rate-related measures and realism-related measures. Lip-sync is essential for applications that require precise audio-visual alignment, focusing on synchronizing audio and lip movements. Realism is important for applications that require high visual fidelity and overall believability of the generated content. It takes into account not only lip synchronization, but also other factors such as facial expressions, eye movements, skin texture, and lighting. Lip-sync rate can be measured using metrics like LSE-C, LSE-D, and LMD, while realism can be measured through PSNR, SSIM, FID, and perceptual human evaluations (such as mean opinion score (MOS) \cite{lu2022visualtts, hou2024polyglotfake}).

\paragraph{BRISQUE}

BRISQUE is an image quality assessment (IQA) model that can evaluate the quality of an image without needing a reference image \cite{mittal2012no}. It works by analyzing natural scene statistics in the spatial domain, directly examining pixel values without transforming the image into a different domain, such as the frequency domain. The model employs statistical features derived from natural scene statistics to capture deviations from natural image properties, indicating distortions and quality degradation. This makes it useful for detecting deepfakes, as it does not rely on a real image for comparison once it's deployed in the world \cite{hou2024polyglotfake, yang2020deepfake}. 


\subsection{Multimodal Deepfake Generation Tools}

\textcolor{black}{A Deepfake Generation Tool is a sophisticated software or system designed to synthesize and create realistic media content across multiple modalities—primarily video and audio. These tools leverage advanced artificial intelligence (AI) and deep learning techniques to generate highly convincing synthetic content, often using generative models like GANs (Generative Adversarial Networks) or diffusion models. Deepfake generation tools can create content that closely mimics real media, making it challenging to distinguish between authentic and synthetic.}

\begin{table*}[htbp]
\caption{Top Tools to Detect Multimodal Deepfakes}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
Method & Free & Open-source & URL\\\hline\hline
Synthesia  & \xmark & \xmark & https://www.synthesia.io/ \\\hline
AI Studios by DeepBrain AI  & \xmark & \xmark & https://www.aistudios.com/ \\\hline
Creative Reality Studio by D-ID  & \xmark & \xmark & https://www.d-id.com/creative-reality-studio/ \\\hline
Elai.io  & \xmark & \xmark & https://elai.io/ \\\hline
\end{tabular}}
\label{tab:tool_det_multimodal_deepfakes}
\end{table*}

\textcolor{black}{The rise of accessible deepfake generation tools has revolutionized content creation in several areas, particularly in Training & Education, E-commerce, Social Media, and Customer Support. These platforms use advanced AI to generate realistic videos based on text prompts, featuring avatars that can speak, express emotions, and perform subtle facial gestures. Designed mainly for professional use, these tools allow users to create customized video content at scale without the need for complex equipment, technical expertise, or high production costs. One of the most notable features of these tools is their user-friendly interface, which enables non-technical users and beginners to quickly produce sophisticated video content. Most of these platforms utilize deep learning and computer vision techniques to animate pre-existing avatars according to user-provided text prompts. The avatars are often photorealistic digital representations of real individuals, providing a high level of realism.}

\subsection{Multimodal Deepfake Detection}
\label{subsec:multimodal_detection}

Multimodal deepfake detection is an important area of research that focuses on identifying synthetic media manipulating multiple modalities, such as video, audio, and text, to create highly realistic and deceptive content \cite{raza2023multimodaltrace, katamneni2023mis, 10081373}. Unlike traditional deepfakes that target a single modality, multimodal deepfakes integrate alterations across several types of data, making them more sophisticated and harder to detect. Detection approaches typically use machine learning and deep learning algorithms, which are trained to recognize subtle anomalies in the synchronized behaviour of different modalities. For example, discrepancies between lip movements and speech, unnatural facial expressions, or inconsistencies in lighting and shadows can signal the presence of a deepfake \cite{lewis2020deepfake}. As deepfake technology continues to evolve, detection methods must also evolve to ensure the integrity and authenticity of digital media in an increasingly digital and interconnected world. In this section, we highlight the latest advancements in multi-modal deepfake detection technology.

\Rotatebox{90}{
\centering
\renewcommand{\arraystretch}{1}
\caption{\textcolor{black}{Multimodal Deepfake Detection Approaches}}
\begin{tabular}{|P{70pt}|P{120pt}|P{120pt}|P{130pt}|P{85pt}|}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Feature Extractors} & \multirow{2}{*}{Technical Novelty} & \multirow{2}{*}{Performance} \\\cline{2-3}
& Audio & Video & & \\\hline\hline
Multimodaltrace \cite{raza2023multimodaltrace} & Resnet-1D on positive frequencies of FFT features & Multilayered 3D ResNet on normalised stacked video frames & Independent and joint feature learning through IntrAmodality Mixer Layer (IAML) and IntErModality Mixer Layer (IEML) & FakeAVCeleb: 92.9\% PDD: 70\% \\\hline
MIS-AVoiDD \cite{katamneni2023mis} & MFCC & MTCNN for face detection and Xception-based for feature extraction & Joint use of modality-invariant and specific representations to ensure both common and unique patterns of real or fake content are preserved and fused &  FakeAVCeleb: 96.2\%(Accuracy) 0.973(AUC) \\\hline
AVoiD-DF \cite{10081373} & transformer network on Mel-spectrograms of audio & transformer network on visual frames & Multimodal temporal \& spatial encoder (TSE) with multimodal joint decoder (MMD)  &  FakeAVCeleb: 83.7\%(Accuracy) 0.892(AUC) \\\hline
PVASS-MDD \cite{yu2023pvass} & VGGish network on log mel-spectrograms of audio \cite{hershey2017cnn} & MTCNN for face extraction and a Swin-Transformer \cite{liu2022video} & Cross-modal predictive VA alignment module  &  FakeAVCeleb: 84.3\%(Accuracy) 0.875(AUC) \\\hline
Emotions Don't Lie \cite{mittal2020emotions} & 13 MFCC features from pyAudioAnalysis \cite{giannakopoulos2015pyaudioanalysis} + DCNNs for modality encoding and perceived emotion encoding & facial features from OpnFace (430-D) \cite{amos2016openface} + DCNNs for modality encoding and perceived emotion encoding & Comparison of affective cues corresponding to perceived emotion to infer whether the video is manipulated & DFDC: 84.4\% \\\hline
AVAD \cite{feng2023self} & \multicolumn{2}{C{160pt}|}{Audio-visual synchronisation model  as in \cite{chen2021audio}. CNN-based feature encoders for visual frames and audio spectrograms and transformer as synchronisation module.} & Video forensics posed as an audio-visual anomaly detection problem and learning only on real videos  &  FakeAVCeleb: 87.9\%(AP) 0.900(AUC) \\\hline
VFD \cite{cheng2023voice} &  \multicolumn{2}{C{160pt}|}{Deep forward convolutional projection on the spectrogram and visual frames + transformer-like network to learn identity-related features} & A face-voice matching technique that measures homogeneity between the audio and video to identify deepfakes  &  FakeAVCeleb: 81.52\%(Accuracy) 0.8611(AUC) DFDC: 80.96\%(Accuracy) 0.8513(AUC)  \\\hline
Capsule Forensics (score fusion) \cite{muppalla2023integrating} & Capsule network on Mel-spectrograms of audio & Capsule network on MTCNN extracted face regions &  Multimodal score-fusion capable of identifying inconsistencies across
various deepfake types and artifacts within each modality  &  FakeAVCeleb: 99.2\%(Accuracy) 0.993(AUC) \\\hline
FCMT + DDIC \cite{liu2023magnifying} &  Audio Forgery Clues Magnification Transformer (FCMT) & Video FCMT &  FCMT module to capture intra-modal artifacts from different modalities by magnifying forgery clues + image spatial artifacts magnification with DDIC  &  FakeAVCeleb: 99.13\%(Accuracy) 0.9927(AUC) DFDC: 98.45\%(Accuracy) 0.9903(AUC)  \\\hline
\end{tabular}
\label{tab:multimodal_detectiondatasets}
}

To effectively detect realistic deepfakes, it is crucial to address both audio and video manipulation. This can be achieved either by independently detecting audio and video cues in deepfakes or through a combined approach that leverages joint audiovisual representation learning. Raza \textit{et al.} \cite{raza2023multimodaltrace} introduced a unified multimodal framework called "Multimodaltrace" which extracts learned feature representations from both audio and visual data, processing these elements separately before integrating them using an innovative multimodal fusion technique. Furthermore, they proposed a novel reformulation of the audiovisual deepfake detection problem, framing it as a multi-label classification task. This new approach predicts confidence levels across both audio and visual modalities, offering a more nuanced and effective method for identifying deepfakes. In their study, Katamneni et al.\cite{katamneni2023mis} focused on fusing modality invariant and specific feature representations for audio and visual streams. This method is similar to previous approaches but employs a different combination of regularization and learning objectives (modality invariant loss, modality-specific loss, and orthogonal loss), leading to improved results. Yang \textit{et al.} \cite{10081373} have proposed an innovative approach for detecting deepfakes by using audio-visual joint learning (AVoiD-DF) which leverages audio-visual inconsistencies for multi-modal forgery detection. The process begins by embedding temporal-spatial information in a Temporal-Spatial Encoder (TSE) to obtain temporal-spatial inconsistency between audio-visual signals (real and fake can exist across frames along the temporal dimension). It is then followed by a Multi-Modal Joint Decoder (MMD) to fuse multi-modal features and learn inherent relationships concurrently. Finally, a Cross-Modal Classifier is developed to detect manipulation by detecting inter-modal and intra-modal disharmony. Furthermore, to test the effectiveness of the proposed deepfake detection model in real-world scenarios, the researchers introduced DefakeAVMiT \cite{10081373}, a multimodal deepfake dataset where various forgery techniques have been applied to different modalities.

In the PVASS-MDD framework proposed by Yu \textit{et al.} \cite{yu2023pvass}, there are two main modules: an auxiliary PVASS stage that focuses on exploring common correspondences between video and audio (AV) and a cross-modal predictive VA alignment module (MDD). The PVASS module works by iteratively predicting audio features using visual features and then reconstructing visual features based on audio features and prediction errors to eliminate discrepancies between video and audio. In the MDD stage, the frozen PVASS network from the first stage is used to align the VA features of real videos, enabling the detection network to better learn the inconsistencies between video and audio in deepfake videos. This MDD stage, with the assistance of PVASS, can extract more accurate VA inconsistencies for multimodal deepfake detection. When it comes to detecting deepfakes, Feng \textit{et al.} \cite{feng2023self} took a different approach compared to other techniques. Instead of treating it as a classification problem, they looked at it as an anomaly detection problem. They analyzed the distribution of audio-visual examples and flagged those with low probability. They focused on subtle properties that manipulated videos are unlikely to accurately capture. They used three unique features for audio-visual anomaly detection: discrete time delay, time-delay distribution, and audio-visual network activations. They found that time-delay distribution is more meaningful for anomaly detection than time-delay alone. They also studied the effect of feature activations within the audio-visual synchronization network on anomaly detection. The results showed that manipulated videos can be detected by identifying unlikely sequences of these features based on a learned distribution. Mittal \textit{et al.} \cite{mittal2020emotions} proposed an innovative method for detecting alterations in videos, such as deepfakes. This approach utilizes both audio (speech) and video (face) data and extracts emotional features from both modalities. The method uses a Siamese network-based architecture (triplet learning) to process real and deepfake videos at the same time during training. It generates modality and perceived emotion embedding vectors for the subject's face and speech, which are then used to distinguish between real and fake content. Through experiments, the study demonstrated that the perceived emotion cues from both modalities play a crucial role in detecting deepfake content by assessing the similarity between modality signals. 

Cheng \textit{et al.} \cite{cheng2023voice} investigated using voice-face matching to detect deepfake videos. Their empirical results indicated that the identities behind voices and faces are often mismatched in deepfake videos and that voices and faces have some level of homogeneity. They detected deepfakes by examining the intrinsic correlation of facial and audio information, without using any additional auxiliary data such as more modalities or visual features. Muppalla \textit{et al.} \cite{muppalla2023integrating} utilised capsule networks to extract robust features from audio spectrograms and face visuals followed by multimodal fusion and classification for deepfake detection. They utilised both score-fusion and feature-fusion approaches, which substantially improved over the state-of-the-art methods. In their recent work, Liu \textit{et al.} \cite{liu2023magnifying} introduced an innovative multimodal Deepfake detection framework that enhances intra-modal and cross-modal forgery clues. The framework consists of several key modules. Firstly, the Forgery Clues Magnification Transformer (FCMT) module is proposed to capture temporal intra-modal defects by magnifying forgery clues based on sequence-level relationships. Additionally, a Distribution Difference Inconsistency Computing (DDIC) module, based on Jensen–Shannon divergence, is used to adaptively align multimodal information for further magnifying the cross-modal inconsistency. The framework also explores spatial artifacts by connecting multi-scale feature representation to provide comprehensive information. Finally, a feature fusion module is designed to adaptively fuse features to generate a more discriminative feature. Experimental results showed that the proposed framework outperforms independently trained models and demonstrated a superior generalisation on unseen types of Deepfake. The overall performance of the selected deepfake detection techniques on FakeAVCeleb dataset \cite{khalid2021fakeavceleb} is illustrated in Figure \ref{fig:multimodal_summary} in terms of accuracy and area under the curve (AUC) score.

\begin{figure}
    \centering
    \includegraphics[width=.5\linewidth]{figures_new/FakeAVCeleb.pdf}
    \caption{\textcolor{black}{Performance variation of recent state-of-the-art methods in detecting deepfakes on FakeAVCeleb dataset in terms of Accuracy and AUC.}}
    \label{fig:multimodal_summary}
\end{figure}

\textcolor{black}{Detecting deepfakes that involve manipulation across multiple types of media is a crucial task, and it is challenging to detect these using single-modal approaches highlighting the importance of addressing both audio and video manipulation in detection. While many methods have been proposed in the literature using different feature extraction and fusion techniques, most of them share similar architectural patterns. However, some state-of-the-art techniques have introduced novel approaches for deepfake detection. These advanced methods analyze audiovisual features iteratively, treating detection as an anomaly detection problem, and identifying inconsistencies using unique features like time-delay distribution and network activations. In addition, leveraging emotional features from both audio and visual sources, along with effective voice and face-matching techniques, greatly improves the chances of identifying deepfakes. More refined techniques also enhance the ability to detect forgery by emphasizing signs of manipulation and aligning the information from different media types. This leads to better performance and accuracy when detecting deepfakes that haven't been seen before. These developments in multimodal deepfake detection provide a more thorough and reliable way to spot manipulated content. Such improvements are essential for maintaining the trustworthiness of digital media and reducing the risks posed by misinformation in our increasingly complex online world.}

\subsection{Multimodal Deepfake Detection Tools}

\textcolor{black}{A Deepfake Detection Tool is an advanced software solution designed to identify and flag manipulated or synthetically generated digital content, including videos, audio, images, and increasingly, text. As deepfake generation techniques have become more sophisticated, detection tools have had to evolve as well, often utilizing state-of-the-art artificial intelligence (AI) and deep learning (DL) methods to keep pace with the capabilities of AI-generated forgeries. These detection tools analyze various features within digital media, employing algorithms that can identify subtle anomalies in pixel patterns, audio signals, or inconsistencies in images and videos that often occur during the deepfake creation process. Such tools not only serve as protective measures for individuals and organizations but are also gaining traction in sectors like law enforcement, cybersecurity, and media integrity, where they help maintain trustworthy sources of information. Table \ref{tab:tool_det_multimodal_deepfakes} provides a comparative overview of several currently available deepfake detection tools.}

\begin{table*}[htbp]
\caption{Top Tools to Detect Multimodal Deepfakes}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
Method & Free & Open-source & URL\\\hline\hline
Sentinel  & \xmark & \xmark & https://thesentinel.ai/ \\\hline
Sensity  & \xmark & \xmark & https://sensity.ai/  \\\hline
Audio Visual Forensics & \cmark & \cmark & https://github.com/cfeng16/audio-visual-forensics \\\hline
Deepware  & \xmark & \xmark & https://deepware.ai/  \\\hline
Reality-Defender  & \xmark & \xmark & https://www.realitydefender.com/ \\\hline
Phoneme-Viseme Mismatch Detector  & \xmark & article & https://ieeexplore.ieee.org/document/9151013 \\\hline
\end{tabular}}
\label{tab:tool_det_multimodal_deepfakes}
\end{table*}


\subsection{Future Trends in Multimodal Deepfake Generation and Detection}

\textcolor{black}{In recent years, the creation of multimodal deepfakes has progressed rapidly, creating an ongoing challenge between making realistic deepfakes and developing methods to detect them. Diffusion models are one recent approach in image generation, which can be adapted for multimedia deepfake creation. These models can manipulate visual features and, when combined with audio signal manipulation techniques, allow for the generation of synchronized, multimodal content that includes both audio and visual modifications \cite{du2024dfadd, firc2024diffuse, av2024latent, bhattacharyya2024diffusion}. Despite the advances in state-of-the-art deepfake generation methods, issues with synchronization across different modalities (such as audio and video) persist. These synchronization inconsistencies are detectable by advanced detection systems and can help identify manipulated content \cite{liz2024generation, ivanovska2024vulnerability, mubarak2023survey}. To improve both deepfake generation and detection methods, high-quality datasets with a wide range of audio and video manipulations are essential. Adding datasets with content from multiple languages (most datasets are currently English-only) and diverse demographic representation would also be beneficial. This would support the development of more robust and generalized generation and detection models. Another key area in deepfake detection is explainability \cite{haq2024multimodal, tsigos2024towards}. Currently, most detection methods rely on deep learning, but what these models specifically learn to distinguish real from fake samples remains unclear. Future research could focus on understanding and interpreting these learning patterns, which could enhance both the effectiveness and trustworthiness of detection systems. In the future, multimodal deepfakes are likely to become increasingly realistic and harder to detect as techniques evolve. This makes it critical for research to keep pace, continually improving both generation and detection methods to address these advancements.}


\subsection{Combating Multimodal Deepfakes in Multimodal Biometrics}
\label{subsec:multimodal_biometrics}
With the advances in biometric evaluation techniques multimodal biometric recognition has also been recently introduced. Therefore, it is important to investigate the ability of multimodal deepfakes, especially the voice and face multimodal systems to thwart multimodal biometric recognition. In the following subsection, we discuss the summary of the findings of our evaluation, and a detailed discussion is provided in Sec. III of supplementary material
\subsubsection{Efficacy of multimodal deepfakes to fool multimodal biometrics systems}
Table III in Sec. III of supplementary material discusses the effectiveness of state-of-the-art multimodal deepfakes to thwart multimodal biometric recognition. Please note that this evaluation was conducted using voice and face multimodal systems and we considered a framework where voice modality and face modality are individually validated biometrically and the final decision is generated by fusing the individual decisions. While the current state-of-the-art multimodal deepfake generation methods failed to thwart the overall framework, especially due to their poor performance in manipulating the voice modality, the advances in multimodal deepfake technology could soon surpass the multimodal biometric reconnection and become a threat to multimodal authentication systems.


\subsubsection{Measures for revealing true identity:} To the best of our knowledge, there is no method to recover true identity from multimodal deepfakes. 



% \newpage

% \subsubsection{Universal multimodal deepfake detectors ? \textcolor{black}{I think this must come under unimodal techniques. Couldn't find any one detector that works on both audio and video. But there are many scenarios with identifying multiple types of attacks using single modality with one network}}

% \hspace{2mm}
% \subsection{Combating multimodal deepfakes in multimodal biometrics}
% \subsubsection{Efficacy of multimodal deepfakes to fool multimodal biometrics systems}
% \subsubsection{Measures for revealing true identity}

==> tex/voice.tex <==
\section{Voice Deepfakes}\label{sec:voice_deepfakes}
%\textcolor{red}{RESPONSIBILITY - Ivan \& Darshana}

\subsection{Generation}\label{sec:voice_generation}

Voice deepfake or synthetic voice is a voice that closely resembles a real person’s voice. It refers to any voice that is generated using artificial intelligence (AI) technology and can accurately capture tonality, accents, cadence, and other unique characteristics of a real person’s voice. Fake voices can be used to create speech sentences that sound like real people saying things they did not say. Human voice synthesis can be broadly classified into text-to-speech (TTS) and voice conversion (VC). Figure~\ref{fig:voice_deepfakes} shows two popular pipelines for creating voice deepfakes.

\subsubsection{Voice Deepfake Types}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures_new/voice_deepfakes.pdf}
    \caption{Two popular methods for creating voice deepfakes: (a) Text-to-speech and (b) Voice conversion. [REDONE]}
    \label{fig:voice_deepfakes}
\end{figure*}

\paragraph{Text-to-Speech (TTS)}

A text-to-speech (TTS) system aims to create speech from a provided input text. Thanks to recent advances in deep learning and artificial intelligence, TTS systems can now produce realistic and natural-sounding speech using any speaker’s voice. Generally, modern TTS systems consist of three basic components \cite{surveytts}: a text analysis module, an acoustic model, and a vocoder. When the user inputs text into the TTS system, a text analysis module processes the text and extracts linguistic features. The acoustic model then generates acoustic features based on the linguistic features. Finally, the vocoder synthesizes speech from the predicted acoustic features. To better capture the characteristics of voices from various speakers, speaker embeddings extracted from the speaker encoder network are commonly used in the acoustic modelling process \cite{jia2018transfer}. In recent years, a transformer with a self-attention mechanism \cite{transformer} has gained widespread popularity as an architecture for acoustic models in neural TTS. Moreover, fully end-to-end models like FastSpeech 2s \cite{ren2021fastspeech}, VITS (Conditional Variational Autoencoder with Adversarial Learning for End-to-End Text-to-Speech) \cite {vits}, and NaturalSpeech \cite{naturalspeech} have been specifically designed to directly generate speech waveforms from character or phoneme sequences, aiming to enhance optimization and reduce development time for various TTS components.

In recent times, Large Language Models (LLMs) have been introduced to improve the quality and speaker adaptation of TTS models even further. LLMs are fundamental machine learning models that are trained with massive amounts of text to understand, predict, and generate human language \cite {surveyllm}. 
For instance, several studies on TTS have utilized Bidirectional Encoder Representations from Transformers (BERT) embeddings to generate speech with improved prosody prediction, better pronunciation and expressiveness \cite{chen2021, kenter2020, xiao2020, xu2021}. Since BERT or BERT-like models learn contextual information from a large-scale text corpus, they can provide syntactic and semantic information to help in predicting the fundamental frequency \cite{yasuda2022}, pauses \cite{xiao2020}, and other prosodic characteristics \cite{moya2023a} of natural speech. The representations from large-scale Self-Supervised Learning (SSL) models such as HuBERT \cite{hsu2021hubert}, WavLM \cite{chen2022wavlm}, and Wav2vec 2.0 \cite{baevski2020wav2vec} are highly beneficial for speech generation tasks. They can be easily adapted to various non-automatic speech recognition tasks, including speaker identification, spoken language understanding, and speech emotion recognition \cite{ftwav2vec}. In the field of TTS, SSL features have been explored in prosody modelling \cite{zhang2023}, improving pronunciation accuracy in cross-lingual TTS \cite{cong2022}, noise-robust synthesis \cite{Siuzdak2022}, and zero-shot TTS \cite{hierspeech,fujita2023}. To achieve superior performance, recent TTS systems such as $\text{M}^{2}$-CTTS \cite{xue2023}, WavThruVec \cite{siuzdak22} and HierSpeech++ \cite{hierspeech} have used SSL representations as an additional semantic representation. StyleTTS2 \cite{styletts2} has also benefited from the SSL model through adversarial training.

The development of Generative Pre-trained Transformers (GPT) technology \cite{gpt} has inspired recent efforts to harness the capabilities of GPT-like auto-regressive models for building large-scale TTS systems. For instance, VALL-E \cite{valle} is the initial neural codec language model designed based on the architecture of GPT-3, featuring robust in-context learning abilities. VALL-E generates the discrete audio codec from phonemes representing the target content and acoustic code prompts extracted from the speaker's voice. It also can produce high-quality personalized voices and emotions based on short speech prompts. Its multilingual variant, VALL-E X \cite{vallex} introduces language ID for synthesizing cross-lingual speech, which supports speech-to-speech translation. LauraGPT (Listen, Attend, Understand, and Regenerate Audio with GPT) \cite{lauratts} adopts a decoder-only Transformer as a GPT backbone to perform unified audio and text modelling and can generate outputs in either modality. Furthermore, Cosyvoice \cite{cosyvoice} and FireRedTTS \cite{fireredtts} introduce semantic speech tokens for TTS modelling and formulate TTS as a next-token prediction task with text as prompts using the GPT-like decoder transformer.

While the auto-regressive model-based architecture has achieved promising results, inference latency is higher compared to non-autoregressive models because the codec token needs to be sampled sequentially for speech generation. Using the text-guided speech-infilling task \cite{le2023voicebox},  E2-TTS \cite{e2tts} and F5-TTS \cite{f5tts} predict masked speech given its surrounding audio and the text transcript in a non-autoregressive manner. During training, the text input is padded with filler tokens of the same length as input speech, simplifying the TTS systems without complex designs such as duration model, text encoder, and phone alignment.  

In voice generation scenarios, providing a text description to describe the intended voice attributes such as speaker identity, tone, speaking rate, and emotion, would be more user-friendly and offer greater voice customization \cite{guo2023, instruct_tts, prompt_tts2}. One notable example is Parler-TTS \cite{lacombe-etal-2024-parler-tts} which utilizes the MusicGen \textcolor{red}{\cite{copet2024simple}} architecture conditioned on embeddings extracted from the Flan-T5 text encoder through a cross-attention mechanism to control different speaker attributes using natural language descriptions \cite{lyth2024natural}.

\paragraph{Voice Conversion (VC)}

Voice Conversion (VC) is the process of transforming a source speaker's voice to sound like that of another speaker without changing the linguistic content. This change alters the speaker identity of the converted speech \cite{hamid2017}. There is a growing demand for various practical applications of VC technology, which can benefit consumers in many ways, such as personalized text-to-speech, voice dubbing, voice mimicry, and speaking aids for speech-impaired persons \cite{kain2007, biadsy2019}. However, VC can also be misused by malicious actors to mimic voices and manipulate what we hear for their advantage.

The VC system pipeline typically consists of three main phases \cite{Sisman2020}: (1) speech analysis and feature extraction phase where the speech from a source speaker is converted into features containing linguistic contents and disentangled from its speaker's characteristics, (2) feature mapping phase where the decomposed information is transferred into intermediate features that match the target speaker's characteristics, and (3) reconstruction phase where the modified intermediate features are transformed back into a speech waveform using a vocoder.
In the parallel voice conversion (VC) technique, the VC system is trained to learn a mapping function from the source speech to the target speech using a training set that contains parallel data. This means that the training set includes speech data of the same linguistic content from both the source and the target speakers \cite{Sisman2020}. However, the requirement for parallel data has often hindered the progress of parallel VC techniques because it is usually assumed that there is a limited amount of data available from both the source and target speakers.  In recent years, deep learning techniques have become increasingly effective in solving conversion problems using a mapping function with powerful regression capabilities, without the need for a parallel corpus (non-parallel VC). VC frameworks such as CyleGAN-VC \cite{cycleganvc}, StarGAN-VC \cite{starganvc}, and VAW-GAN \cite{vawgan} have been developed by incorporating generative adversarial networks to map various voice attributes. These techniques can achieve better voice quality and similarity to the target speaker when a large number of training examples are available.

The use of linguistic-related features to capture spoken content has been a popular approach for non-parallel VC \cite{flytek2018, tian2019}. These features can be derived from an Automatic Speech Recognition (ASR) system, such as bottleneck features or Phonetic PosteriorGrams (PPGs) \cite{ppg2016}. A PPG is a matrix that represents the posterior probabilities of the phonetic class corresponding to each time frame. It is common to employ speaker-independent ASR (SI-ASR) trained using a large multi-speaker corpus to obtain PPGs to accommodate for differences in speakers. Recently, large-scale self-supervised speech representations such as wav2vec 2.0, vq-wav2vec \cite{baevski2019vq}, HuBERT and WavLM have been used to replace the PPGs in voice conversion tasks \cite{polyak2021, huang2022, li2023freevc}. For instance, Free-VC \cite{li2023freevc}, an end-to-end model based on the VITS architecture designed for voice conversion, has used WavLM to encode linguistic content. Speaker information is acquired from a speaker encoder trained jointly with the rest of the components from scratch. Additionally, SR-based data augmentation is employed to enhance the quality of waveform generation.

Although continuous features extracted from self-supervised pre-trained models can capture linguistic, speaker, prosodic, and semantic information of speech, it remains a challenge to completely separate the content from the speaker identity, resulting in reduced speaker similarity of the converted speech. There are multiple methods in the literature that can be applied to SSL continuous features such as discretization \cite{polyak2021, softvc}, and speaker disentanglement mechanisms \cite{contentvec}. For example, ContentVec \cite{contentvec} introduces disentanglement modules in the mask prediction task of HuBERT without significant loss of content information. The content encoder in \cite{softvc} produces soft speech units, called HuBERT-Soft, which are learned by predicting a distribution over the discrete units extracted from HuBERT to achieve speaker disentanglement. These HuBERT-Soft features have been widely employed as content features in voice conversion tasks \cite{quickvc, rythmvc, streamvc}, including singing voice conversion \cite{singingvc, diffsvc}, and have notably improved speaker similarity.

%The method in~\cite{softvc} is proposed to apply k-means on the continuous features to generate discrete speech units as a mean to improve the speaker similarity.

\subsubsection{Deepfake Generation Process} 

\paragraph{Autoregressive Models}

The autoregressive model predicts the model behaviour of the current step using the data in the previous time steps. For example, in a linear autoregressive model of order $n_i$, the output $y[t]$ can be estimated by:

\begin{equation}
y[t] = \sum^{n_i}_{i=1} a_{i}x[t-i] + e[t]
\end{equation}

where $a_{i}$ is the model parameters, $e[t]$ is white noise or residual error with zero mean. In deep autoregressive models, the model parameters are estimated using deep neural networks. The dependency modelling of an input data sequence in an autoregressive manner allows the complex structure of data to be learned in a temporally more coherent way. However, an autoregressive model suffers from slow generation because it depends on the previous observations to predict the value at the current time step. 

Autoregressive structures have been adopted in many neural TTS systems to achieve state-of-the-art performance such as Tacotron 1/2 \cite{tacotron, tacotron2}, DurIAN \cite{durian}, and DeepVoice 3 \cite{deepvoice3}. One of the first neural-based vocoders for speech synthesis is WaveNet \cite{wavenet}. The autoregressive structure of WaveNet improves the continuity of the generated waveform because it generates one sample at a time.

\paragraph{Variational Autoencoders}

Variational Autoencoders (VAE) consist of an encoder that encodes input data $x$ into a regularized multivariate latent distribution \textcolor{red}{$q(z|x)$}, and a decoder that reconstructs the data as accurately as possible by sampling a point from this distribution \textcolor{red}{$z \sim q(z|x)$}. The decoder and encoder in VAE are trained to minimize the construction error, which also adds a regularization term in the loss function. This term ensures that the latent distribution is regularized to some prior distribution, usually multivariate Gaussian, during training.

In the neural network-based TTS model, the VAE is used to compress the high-dimensional speech $x$ into frame-level representations $z$, where $z$ is sampled from the posterior distribution $q(z|x)$. It is assumed that the prior $p(z)$ is the standard isotropic multivariate Gaussian. Given $q(z|x)$, the speech waveform is reconstructed from $p(x|z)$ using a decoder. In VITS \cite{vits, naturalspeech}, the $z$ is predicted from phoneme sequence $y$, where $z$ is sampled the predicted prior distribution, $p(z|y)$. To enable the speech synthesis, the VAE and the prior prediction are jointly optimized with the loss function consists of a waveform reconstruction loss -log $p(x|z)$ and a Kullback-Leibler divergence loss between the posterior $q(z|x)$ and the prior $p(z|y)$, $KL[q(z|x)||p(z|y)]$.

%The VAE has been used as the key component in many neural network based TTS models.

\paragraph{Generative Adversarial Networks}

Generative Adversarial Networks (GANs) are generative models that create new data instances with the same underlying data distribution of the training samples. GANs generate an N-dimensional vector from an N-dimensional random vector sampled from a simple distribution (standard Gaussian). Because of the complexity of data distribution, GANs formulate this problem into a game between two neural networks that compete against each other to reach a zero-sum Nash equilibrium profile~\cite{Goodfellow2014}. The generator network aims to produce synthetic output based on the target's data distribution to fool the discriminator. Meanwhile, the discriminator network aims to differentiate whether the generated sample is real or fake by comparing the output with the true data.

GAN has been widely used to train a neural vocoder for synthesizing high-fidelity speech audio. Typical non-autoregessive neural vocoders such as~\cite{melgan, hifigan, parallelgan} employ a generator and a sets of discriminators which are trained adversarially using GAN losses to model raw waveforms.

\paragraph{Normalizing Flows}

Normalizing flows employs a sequence of invertible and differentiable mappings, referred as the flow, that transform a simple probability distribution (e.g., standard Normal) into a more complex distribution.

To generate data points $\boldsymbol{x}$ that follow the distribution we want to generate, one can sample $\boldsymbol{z}$ from the base distribution (the “noise”) $p_{\theta}(\boldsymbol{z})$ of a zero mean spherical Gaussian, $p_{\theta}(\boldsymbol{z}) = \mathcal{N}(\boldsymbol{z};0,\boldsymbol{I})$. This process can be written as,
\begin{equation}
   \boldsymbol{z} \sim \mathcal{N}(\boldsymbol{z};0,\boldsymbol{I})
\end{equation}
\begin{equation}
   \boldsymbol{x} = \boldsymbol{f}_{1} \circ \boldsymbol{f}_{2} \circ \ldots \boldsymbol{f}_{K} %(\bm{z})
\end{equation}
where $\boldsymbol{x}$ can be generated by progressively transforming a random variable ($\boldsymbol{z}$) using a set of K invertible  functions, i.e., bijective. The flow-based model is trained by maximizing the log likelihood of the model parameters given the data $\boldsymbol{x}$ based on a change of variable rules,
\begin{equation}
    \log p_{\theta}(\boldsymbol{x}) = \log p_{\theta}(\boldsymbol{z}) + \sum_{i=1}^{K} \log |\det(\boldsymbol{J}(\boldsymbol{f}_{i}^{-1}(\boldsymbol{x})))|
    \end{equation}
\begin{equation}
    \boldsymbol{z} = \boldsymbol{f}_{K}^{-1} \circ \boldsymbol{f}_{k-1}^{-1} \circ \ldots \boldsymbol{f}_{0}^{-1}(\boldsymbol{x})
\end{equation}
where $\boldsymbol{J}$ denotes the Jacobian matrix of $\boldsymbol{f}_{i}^{-1}$, and $\det(.)$ is the the determinant of the matrix.

In a flow-based vocoder such as WaveGlow~\cite{waveglow}, the invertible mapping is constructed using an affine coupling layer~\cite{realnvp}. Each flow operation consists of invertible $1 \times 1$ convolution followed by an affine coupling layer. %Normalizing flow has been adopted for speech synthesis, but the implementation usually require large number of model parameters to improve the quality of synthesis~\cite{}. 
In TTS, Flowtron model~\cite{flowtron} is based on autoregressive flow that generates a sequence of mel spectrogram frames conditioned on text and speaker embedding. Flowtron provides control over speech variation and expressiveness and allows for style transfer.


%Some vocoders such as WaveGlow has been using GLOW ..


\paragraph{Denoising Diffusion Probabilistic Models}

Denoising Diffusion Probabilistic Models (DDPMs) encompass two interconnected processes: a forward process that maps the data distribution to a simple prior distribution, typically a Gaussian, and a reverse process that gradually reverse the effect of forward process using neural networks by simulating Ordinary or Stochastic Differential Equations.

Recently, DDPMs have become popular approach for audio generation including TTS. In TTS tasks, the diffusion model has been applied to the acoustic models and also to the vocoders. For example, the acoustic model in Diff-TTS~\cite{diff-tts} and Grad-TTS~\cite{grad-tts} generate Mel-spectrogram from the text with DDPM. In diffusion-based vocoders, DDPMs turn random noise into a high-fidelity speech waveform through an iterative sampling process after hundreds of iterations. The quality of neural vocoders based on DDPMs has been shown to be comparable with AR models~\cite{wavefit}. WaveGrad is one of the earliest work for conditional model waveform generation by combining the score matching and diffusion probabilistic models~\cite{wavegrad}. Another neural vocoder based on diffusion model is DiffWave~\cite{diffwave}. DiffWave is non-autoregressive model, conditioned on Mel-spectrogram. 

% https://arxiv.org/pdf/2303.13336.pdf

\subsubsection{Performance Evaluation}

% https://www.mdpi.com/2079-9292/9/2/267
% https://www.sciencedirect.com/science/article/pii/S0885230803000676

The quality of synthetic speech is typically evaluated using subjective and objective assessments. Subjective tests involve human listeners rating audio segments based on naturalness and intelligibility~\cite{king2014, electronics20}. Naturalness includes pleasantness, ease of listening, and audio flow, while intelligibility covers listening effort, pronunciation, articulation, comprehension, and speaking rate~\cite{articlemos}. These features are usually evaluated using a mean opinion score (MOS) on a Likert scale from 1 to 5, defined in the recommended standard ITU-T P.85, 1994 for the evaluation of voice output systems~\cite{itu_p85}.

The process of conducting a listening test can be both expensive and time-consuming. It requires a large number of participants who speak the native language or reside in specific geographical areas in order to obtain credible results. In recent years, deep learning models like AutoMOS~\cite{automos}, MOSNet~\cite{mosnet}, and LDNet~\cite{ldnet} have been developed to automatically predict the MOS of synthetic speech, which is highly correlated with human subjective ratings. For the MOS evaluation of multilingual speech synthesis, a Speech Quality Identification (SQuID) system based on multilingual Speech and Language Model (mSLAM) has been designed to predict speech naturalness ratings from 65 different locales~\cite{squid}. Additionally, objective metrics such as Mel-Cepstral distortion (MCD)~\cite{mcd} and word error rate (WER) are often used in combination with subjective tests to measure the quality and intelligibility of synthetic speech.

%The latest work is using regression method: 
%https://arxiv.org/pdf/2210.06324.pdf

\subsubsection{Summary of voice deepfake generation types and methods}

Text-to-speech and voice conversion are the two popular methods for generating fake speech samples. The progress has advanced rapidly with the introduction of an autoregressive GPT-like models, and when self-supervised speech representation learning models are utilised in the training process. Moreover, high-quality samples achieving human parity speech are produced when diffusion probabilistic models are used in the TTS's acoustic modeling. Flow matching~\cite{lipman2023flow}, a recent paradigm in generative modeling that combine aspects from continuous normalizing flows (CNFs) and diffusion models (DMs) to transform between noise and data samples by learning the probability path via ordinary differential equation (ODE) has shown superior modeling performance with stable and faster training. For example, Macha-TTS~\cite{matcha2024}  use optimal-transport conditional flow matching to train an encoder-decoder TTS model. Meanwhile, VoiceFlow~\cite{voiceflow} employs a rectified flow matching in TTS to achieve superior sample quality with a few number of sampling steps. %which is a new way to synthesize faster and higher quality samples by learning ordinary differential equations to sample from the data distribution.

\hspace{2mm}
\subsection{Detection}\label{sec:voice_detection}
\subsubsection{Features used for deepfake detection} %-> THEY ARE COMBINED/PART OF the literature review on voice deepfake detection


An audio spoofing attack occurs when an attacker creates a fake recording of someone's voice to bypass an automatic speaker verification (ASV) system. Although the fake recording may sound like a genuine human person to a human ear, it may still contain certain peculiarities or artifacts that can help in distinguishing it from genuine recordings. To protect the ASV system, voice spoofing countermeasure solutions are usually employed as a first defense mechanism to discriminate between bonafide (genuine) speech and spoofed speech generated using voice deepfake tools. Only bonafide speech will be fed into the ASV system.

A countermeasure system consists of two main modules, a feature extractor and a classifier. Feature selection and extraction play integral parts in spoofing detection algorithms. The features are engineered to be more compact and less redundant compared to the original audio signal. The detection model can also combine model outputs from different types of features to create a fusion model for improved spoofing detection performance~\cite{balamurali2019}.

\paragraph{Techniques based on hand-crafted features}

\textbf{Short-term Cepstral features:}
Mel-Frequency Cepstral Coefficients (MFCCs)~\cite{mfcc} are arguably the most commonly used features as a baseline in speech spoofing detection~\cite{sahidullah2015}. The extraction process of MFCCs begins with computing the power spectrum on each frame of audio signal using a short-time Fourier transform (STFT). Next, triangular filter bank, on a Mel-scale are applied to the power spectrum to extract frequency bands. Mel-scale aims to mimic the perceptually relevant aspects of human hearing, by being more discriminative at lower frequencies and less at higher frequencies. The logarithm of magnitude spectrum is then computed and followed by applying discrete cosine transform (DCT) to decorrelate the filter bank energies. Typically in speech recognition, 13 coefficients of Cepstral values, from the second to the fourteenth, are taken to represent the information regarding the vocal tract features. In practice, it is often to calculate the dynamic values such as delta and acceleration coefficients from the static Cepstral values to take into account the temporal changes in speech from frame to frame.

\textbf{Cepstral features related to MFCCs:}
Different types of filter bank can be used when integrating the power spectrum to compute the Cepstral coefficients. For example, in rectangular filter cepstral coefficients (RFCCs)~\cite{alegre2013}, the integration is performed using a rectangular window, spaced in linear scale. While the linear frequency cepstral coefficients (LFCCs) uses triangular filter bank, spaced in linear frequency scale~\cite{hasan2013}. On the other hand, the IMFCC is produced using the filters that are linearly spaced on the "inverted-mel" scale to put emphasis on the high frequency region~\cite{chakroborty2007}.

\textbf{Constant Q Cepstral Coefficients (CQCCs):}
The constant Q cepstral coefficients (CQCCs) are introduced for the first time as a spoofing countermeasure for automatic speaker verification~\cite{Todisco2017}.  
The CQCCs are obtained by applying time-frequency analysis on speech signal using the constant Q transform (CQT)~\cite{Youngberg1978} followed by the Cepstral analysis.
The CQT provides a greater frequency resolution for lower frequencies and a higher time resolution at higher frequencies, unlike the short-time Fourier transform which
gives constant time and frequency resolution. The resolution of the CQT features captures small variations in lower frequencies which are more useful to the task of spoofing detection.

\textbf{Short-term Phase Features:}
Other researchers have also investigated the use of phase information for speech spoofing detection. For example, some speech synthesis methods cause the loss or phase distortion during the analysis-synthesis steps that can be detected from the phase structure of the speech signals. Phase-based features such as relative phase shift (RPS)~\cite{sanchez2015} which contain purely phase information, modified group delay (MGD)~\cite{wu2012}, and modified relative phase (MRP)~\cite{wang2017} have been shown to be used successfully in the detection of synthetic speech and voice conversion based attacks~\cite{saratxaga2016}.

\subsubsection{Literature review on voice deepfake detection}

%The RPS representation uncovers the phase structure of
%the speech, which is not apparent from the instantaneous
%phase.

\paragraph{Techniques based on learned feature representation}
The conventional method for discriminating bonafide speech from spoofed speech is to train binary classifiers using hand-crafted features. Integrating multiple feature parametrisation is often necessary to improve anti-spoofing performance, for example via score fusion of subsystems based on different features to capture complementary information~\cite{zwu2017}.
Instead of using handcrafted features which are fixed and not learnable, relevant features for discrimination can be learned directly from raw waveform using deep learning techniques. The learnable front-ends can be categorized into two~\cite{fastaudio}: Short-Time Fourier Transform (STFT) based front-ends and First-order Scattering Transform (FST) based front-ends. In STFT based front-ends such as DNN-FBCC~\cite{dnn-fbank} and FastAudio~\cite{fastaudio}, the learned filterbank matrix are multiplied with the a spectrogram to create compressed representations.  For spoof detection task, FastAudio is shown to perform better than handcrafted CQT features and FTS-based front-ends on the ASVspoof 2019 dataset~\cite{fastaudio}.

The FST-based front-end approaches use a convolutional neural network to learn filtering process on raw audio waveform. 
%For example, ~\cite{} uses 
One example of FST-based front-ends is SincNet~\cite{sincnet}, an end-to-end neural network architecture comprises %parameterized Sinc functions as filters in the first layer followed by convolutional layers. 
learnable a bank of band-pass filters parameterized in the form of Sinc functions. SincNet encourages the network to discover more meaningful filters from temporal signal, learning a customized filter bank structure specifically tuned for the desired application. 
RawNet2 combines SincNet and RawNet1 architectures for end-to-end antispoofing~\cite{tak2021}. The first layer of RawNet2 follows the SincNet architecture and the upper layers consist of the same residual networks and GRU layer as RawNet1. RawNet1 is aimed to directly model raw waveforms for the extraction of speaker embedding using convolutional and recurrent neural networks~\cite{jung2019RawNet}. 

To take advantage of the vocoder artifacts in fake audio signals, ~\cite{sun2023} incorporates a vocoder identification module with the feature extractor of the RawNet2. The proposed multi-task learning framework combines multi-class classification loss to classify the type of vocoders used to synthesize fake audio, and a binary classifier to discriminate real from fake. 

\paragraph{Techniques based on self-supervised learning models for speech representations}

Feature extractors using self-supervised learning models for speech representations such as wav2vec and HuBERT have also been investigated for spoofing detection~\cite{xie2021, lantingli2023, kang2024}. The aim is to improve the generalization of the model to unknown attacks rather than using the traditional acoustic features. For example in~\cite{kang2024}, the pretrained wav2vec 2.0 is utilized as a feature extractor, in which several transformer layers are fine-tuned for spoofing countermeasure systems. It is shown that the fine-tuning of the SSL models can result in better generalised spoofing detection performance. Moreover,~\cite{hemlata2023} report the lowest EER for the ASVspoof 2021 logical access (LA) database when using wav2vec 2.0 front-end with the self-attentive aggregation layer and data augmentation strategy.   


%
%\subsubsection{Learning objective and loss functions}
\subsubsection{Performance evaluation}

Voice deepfake detection is primarily treated as a binary classification problem where the task of a countermeasure is to discriminate between bonafide and spoofed utterances. There are two types the binary classifier makes: \textit{false alarms} (false positive), where the classifier accepting spoofed speech that should have been rejected, and \textit{misses} (false negative), where the classifier rejects bonafide speech that should have been accepted. The \textit{false alarm rate} $P_{fa}$ and \textit{miss rate} $P_{miss}$ can be estimated by dividing the number of misses and false alarms by the number of spoof trials and bonafide cases, respectively~\cite{bonastre2021}. 
The most common metric adopted for binary classification is \textit{equal error rate} (EER), a single number in which the \textit{false alarms rate} and the \textit{miss rate} are equal. Lower EER points to a more reliable classifier. However, the EER metric does not consider the level of importance between the $P_{fa}$ and $P_{miss}$, for example when false alarms can be more tolerated than misses.

To suit real-world applications, different cost and class prior parameters are introduced in ASVSpoof 2019 and 2021 to take into account both countermeasure and ASV subsystems as a tandem system, called tandem detection cost function (t-DCF)~\cite{yamagishi:hal-03360794}. The t-DCF is defined as:
\begin{equation}
\text{t-DCF} = 
    \min\limits_{\tau}  \{C_o + C_1P_{miss}(\tau) + C_2 P_{fa}(\tau)\}
\end{equation}
where $P_{miss}$ and $P_{fa}$ are miss and false alarm rates of a countermeasures using a threshold $\tau$, and $C_{0}$, $C_{1}$ and $C_{2}$ are pre-defined cost function parameters that depend on ASV performance as well.
%\subsubsection{Universal deepfake detectors ?}

\hspace{2mm}
\subsection{Combating voice deepfakes in voice biometrics}

Deepfakes pose a significant threat to voice biometrics systems. Using commercial tools, attackers can synthesize the speech of any person to fool speaker recognition systems. For example~\cite{BILIKA2024} found that voice assistants such as Google’s Assistant and Apple’s Siri can be easily tricked using synthesized samples of victims' speech commands,  in which they used an open source "Real Time Voice Cloning" project~\cite{jeremy2019} to clone the voice of the authorized users. As such, it is necessary to evaluate the efficacy of the state-of-the-art voice deepfake generation methods to fool advanced voice biometric systems. In the following subsection, we provide a summary of our evaluation results. For a detailed discussion please refer to Sec. I of supplementary material.

\subsubsection{Efficacy of voice deepfakes to fool voice biometrics systems}
The evaluations presented in Tab. 1 of the supplementary material illustrate that the state-of-the-art speaker recognition system can be vulnerable to off-the-shelf,  publicly available voice deepfakes generation software. As such, there is a pertinent need to upgrade the safety of the existing voice biometrics models against voice deepfakes. 

\subsubsection{Measures for revealing true identity} To the best of our knowledge, currently, there is no method to extract the true identity of a subject when the speech is manipulated using the voice deepfakes method.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\caption{Top ten AI voice cloning tools to create voice deepfakes.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\multicolumn{1}{c}{\multirow{2}{*}{Tools}} & \multicolumn{3}{c}{Features}                                                                                   & \multicolumn{1}{c}{\multirow{2}{*}{URL}} \\
\multicolumn{1}{c}{}              & Used a cloned voice for TTS & Customize pitch/style & Open-source & \multicolumn{1}{c}{}                     \\ \hline \hline
MetaVoice-1B & \cmark & \xmark & \cmark & https://github.com/metavoiceio/metavoice-src \\ \hline
XTTS-v2 & \cmark & \xmark & \cmark & https://github.com/coqui-ai/tts \\ \hline
Soft-VC VITS & \xmark & \cmark & \cmark & https://github.com/svc-develop-team/so-vits-svc \\ \hline
Tortoise-TTS & \cmark & \xmark & \cmark & https://github.com/neonbjb/tortoise-tts \\ \hline
OpenVoice & \cmark & \cmark & \cmark & https://github.com/myshell-ai/OpenVoice \\ \hline
VoiceCraft~\cite{peng2024voicecraft} & \cmark & \xmark & \cmark & https://github.com/jasonppy/VoiceCraft \\ \hline
ElevenLabs     &    \cmark    &    \xmark   & \xmark   & https://elevenlabs.io/                   \\ \hline
Descript       &     \cmark                                   &     \xmark                       & \xmark   &https://www.descript.com/                \\ \hline
Respeecher     &   \cmark                                     &           \cmark                 & \xmark   &https://www.respeecher.com/              \\ \hline
Play.ht   &    \cmark                                    &      \xmark                      & \xmark   &https://play.ht/                         \\ \hline
%Resemble AI  &   \cmark                                     &     \xmark                       & \xmark   &https://www.resemble.ai/       \\ \hline
\end{tabular}}\hspace{2mm}

\end{table*}

